Formal Contact Categories

To each oriented surface S, we associate a differential graded category Ko(S). The homotopy category Ho(Ko(S)) is a triangulated category which satisfies properties akin to those of the contact categories studied by K. Honda. These categories are also related to the algebraic contact categories of Y. Tian and to the bordered sutured categories of R. Zarev.

==> final submit/mymacros.tex <==
\newcommand{\co}{\colon\thinspace}
%\renewcommand{\op}[0]{\normaltext{op}}

%% \usepackage{xparse}
%% \NewDocumentCommand{\raisedminus}{m}{%
%%   \raisebox{0.2em}{$\m@th#1{-}$}%
%% }
%% \NewDocumentCommand{\unaryminus}{}{%
%%   \mathbin{%
%%     \mathchoice{%
%%       \raisedminus\scriptstyle
%%     }{%
%%       \raisedminus\scriptstyle
%%     }{%
%%       \raisedminus\scriptscriptstyle
%%     }{%
%%       \raisedminus\scriptscriptstyle
%%     }%
%%   }%
%% }

%\renewcommand{\DeclareMathOperator}[2]{\DeclareMathOperator{#1}{\bf\ensuremath{#2}}}



% \DeclareMathOperator{\Hm}{H}
% \DeclareMathOperator{\Td}{Td}
% \DeclareMathOperator{\FGL}{FGL}
% \DeclareMathOperator{\Der}{D}
% \DeclareMathOperator{\Deriv}{Der}
% \DeclareMathOperator{\perf}{perf}
% \DeclareMathOperator{\Bimod}{Bimod}
% \DeclareMathOperator{\im}{im}

% \DeclareMathOperator{\Iso}{Iso}
% \DeclareMathOperator{\In}{In}
% \DeclareMathOperator{\Out}{Out}
% \DeclareMathOperator{\Extra}{Extra}
% \DeclareMathOperator{\Hty}{Ho}

% \DeclareMathOperator{\Tout}{Tout}
% \DeclareMathOperator{\Tin}{Tin}


% %\DeclareMathOperator{\Grpoid}{Grpoid}
\DeclareMathOperator{\BBar}{Bar}
% \DeclareMathOperator{\Cobar}{Cobar}
% \DeclareMathOperator{\Hoc}{Hoch}
% \DeclareMathOperator{\Ho}{Ho}
% \DeclareMathOperator{\tr}{Tr}
% \DeclareMathOperator{\Har}{Harr}
% \DeclareMathOperator{\Torus}{Torus}
% \DeclareMathOperator{\Gr}{Gr}

% \DeclareMathOperator{\Cob}{Cob}
% \DeclareMathOperator{\PCob}{Pre-Cob}
% \DeclareMathOperator{\Inj}{Inj}

% %\DeclareMathOperator{\Ab}{Ab}
% \DeclareMathOperator{\Trees}{Trees}
% \DeclareMathOperator{\Tr}{Tr}
% \DeclareMathOperator{\SC}{SC}
% \DeclareMathOperator{\GL}{GL}
% \DeclareMathOperator{\SL}{SL}
% \DeclareMathOperator{\BSL}{BSL}
% \DeclareMathOperator{\img}{im}
% \DeclareMathOperator{\hS}{hS}
% \DeclareMathOperator{\diam}{diam}
% \DeclareMathOperator{\spn}{span}
% \DeclareMathOperator{\Spec}{Spec}
% %\DeclareMathOperator{\Spectra}{Spectra}
% \DeclareMathOperator{\sgn}{sgn}
% \DeclareMathOperator{\Val}{val}
% \DeclareMathOperator{\Alg}{Alg}
% \DeclareMathOperator{\sign}{sgn}
% \DeclareMathOperator{\mcg}{mcg}
% %\DeclareMathOperator{\Lie}{L}
% %\DeclareMathOperator{\Ass}{A}
% %\DeclareMathOperator{\Comm}{C}
% \DeclareMathOperator{\Tw}{Tw}
% \DeclareMathOperator{\Cov}{Cov}
% %\DeclareMathOperator{\Set}{Set}
% %\DeclareMathOperator{\Ring}{Ring}
% %\DeclareMathOperator{\Scheme}{Sch}
% %\DeclareMathOperator{\Sch}{Sch}
% %\DeclareMathOperator{\Aff}{Aff}
% %\DeclareMathOperator{\PStacks}{PStacks}
% %\DeclareMathOperator{\Stackify}{Stackify}
% %\DeclareMathOperator{\Stack}{Stacks}
% %\DeclareMathOperator{\Stacks}{Stacks}
% \DeclareMathOperator{\SSet}{sSet}
% \DeclareMathOperator{\GSet}{GrSet}
% \DeclareMathOperator{\Free}{Free}
% \DeclareMathOperator{\Stab}{Stab}
% %\DeclareMathOperator{\Operad}{Operad}
% \DeclareMathOperator{\Forget}{Forget}
% %\DeclareMathOperator{\Group}{Group}
% %\DeclareMathOperator{\Groups}{Groups}
\DeclareMathOperator{\colim}{colim}
% %\DeclareMathOperator{\grph}{Graph}
% \DeclareMathOperator{\rtree}{RTree}
% \DeclareMathOperator{\tree}{Tree}
% \DeclareMathOperator{\trace}{tr}
% \DeclareMathOperator{\Endo}{End}
% %\DeclareMathOperator{\Ind}{Ind}
% \DeclareMathOperator{\Res}{Res}
% \DeclareMathOperator{\Fgt}{Forget}
% \DeclareMathOperator{\qisms}{qisms}
% \DeclareMathOperator{\Star}{St}
% \DeclareMathOperator{\Auto}{Aut}
% \DeclareMathOperator{\Diff}{Diff}
% %\DeclareMathOperator{\Cat}{Cat}
% %\DeclareMathOperator{\fCat}{fCat}
% %\DeclareMathOperator{\Fuk}{Fuk}
% \DeclareMathOperator{\Isom}{Isom}
% %\DeclareMathOperator{\Coker}{coker}
% %\DeclareMathOperator{\Top}{Top}
% \DeclareMathOperator{\Ker}{ker}
% \DeclareMathOperator{\Orbi}{Orbi}
% \DeclareMathOperator{\Ori}{Or}
% \DeclareMathOperator{\Chain}{Ch}
% %\DeclareMathOperator{\Op}{Operad}
% \DeclareMathOperator{\Coop}{Cooperad}
% %\DeclareMathOperator{\Vect}{Vect}
% \DeclareMathOperator{\HTop}{HTop}
% %\DeclareMathOperator{\Kom}{Kom}
% %\DeclareMathOperator{\Sym}{Sym}
% \DeclareMathOperator{\Ann}{Ann}
% \DeclareMathOperator{\Pos}{Pos}
% \DeclareMathOperator{\Mat}{Mat}
% \DeclareMathOperator{\Bij}{Bij}
% \DeclareMathOperator{\Morph}{Hom}
% %\DeclareMathOperator{\lhom}{hom}
% \DeclareMathOperator{\Fun}{Fun}
% \DeclareMathOperator{\Mor}{Mor}
% \DeclareMathOperator{\Cone}{Cone}
% \DeclareMathOperator{\Inv}{Inv}
% \DeclareMathOperator{\inv}{inv}
% %\DeclareMathOperator{\Homeo}{Homeo}
% %\DeclareMathOperator{\Hom}{Hom}
% %\DeclareMathOperator{\End}{End}
% \DeclareMathOperator{\Aut}{Aut}
% \DeclareMathOperator{\Hpty}{Htpy}
% \DeclareMathOperator{\BHpty}{BHpty}
% \DeclareMathOperator{\ffix}{fix}
% \DeclareMathOperator{\Rp}{Re}
% \DeclareMathOperator{\D}{D}
% %\DeclareMathOperator{\PSh}{PSh}
% %\DeclareMathOperator{\Sh}{Sh}
% %\DeclareMathOperator{\Obj}{Ob}
% %\DeclareMathOperator{\Ob}{Ob}
% \DeclareMathOperator{\rank}{rank}
% \DeclareMathOperator{\Img}{img}
% \DeclareMathOperator{\Pnt}{point}
% \DeclareMathOperator{\Univ}{U}
% \DeclareMathOperator{\TL}{TL}
% \DeclareMathOperator{\BMW}{BMW}
% \DeclareMathOperator{\K}{K}
% \DeclareMathOperator{\G}{G}
% \DeclareMathOperator{\KF}{\FK}
% \DeclareMathOperator{\CKF}{\CFK}
% \DeclareMathOperator{\CFK}{CFK}
% \DeclareMathOperator{\FFK}{RFK}
% \DeclareMathOperator{\HP}{HP}

% \DeclareMathOperator{\Bicat}{Bicat}
% \DeclareMathOperator{\iBicat}{iBicat}


% \DeclareMathOperator{\FK}{FK}
% \DeclareMathOperator{\SU}{SU}
% \DeclareMathOperator{\SO}{SO}
% %\DeclareMathOperator{\Tot}{Tot}
% \DeclareMathOperator{\Hom}{Hom}
% \DeclareMathOperator{\Ktheory}{K}
% \DeclareMathOperator{\Homology}{H}

% \DeclareMathOperator{\Ext}{Ext}
% \DeclareMathOperator{\Tor}{Tor}

% \DeclareMathOperator{\NH}{NH}
% \DeclareMathOperator{\GNH}{GNH}

\newcommand{\uli}[1]{\underline{\smash{\normaltext{#1}}}}
\newcommand{\conj}[1]{\quad\textnormal{ #1 }\quad}
\newcommand{\conjj}[1]{\ \textnormal{ #1 }\ }

\newcommand{\RFlag}[0]{\ensuremath{\RR\!\Flag}}
\newcommand{\RHom}[0]{\ensuremath{\RR\!\Hom}}
\newcommand{\RGamma}[0]{\ensuremath{\RR\!\Gamma}}

\newcommand{\inp}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\inpp}[1]{\ensuremath{\langle\langle #1 \rangle\rangle}}
\newcommand{\inpr}[1]{\left( \ensuremath{ #1 } \right)}

\newcommand{\bmodule}[0]{\operatorname{-}}
\newcommand{\module}[0]{\operatorname{-mod}}
%\newcommand{\alg}[0]{\operatorname{-alg}}
\newcommand{\rmodule}[0]{\operatorname{mod-}\!}
\newcommand{\bimodule}[0]{\operatorname{-mod-}}
\newcommand{\fmodule}[0]{\operatorname{-fmod}}
\newcommand{\gmodule}[0]{\operatorname{-gmod}}
\newcommand{\gfmodule}[0]{\operatorname{-gfmod}}
\newcommand{\gpmodule}[0]{\operatorname{-gpmod}}
\newcommand{\gpfmodule}[0]{\operatorname{-gpfmod}}
%% \newcommand{\stabmodule}[0]{\operatorname{-\underline{mod}}}
%% \newcommand{\stabfmodule}[0]{\operatorname{-\underline{fmod}}}
\newcommand{\stabmodule}[0]{\operatorname{-\uli{mod}}}
\newcommand{\stabfmodule}[0]{\operatorname{-\uli{fmod}}}
\newcommand{\stabFgt}[0]{\operatorname{\uli{Forget}}}

\newcommand{\pmodule}[0]{\operatorname{-pmod}}
\newcommand{\pfmodule}[0]{\operatorname{-pfmod}}
%%\newcommand{\stabgmodule}[0]{\operatorname{-\underline{gmod}}}
%%\newcommand{\stabgfmodule}[0]{\operatorname{-\underline{gfmod}}}
%%\newcommand{\gstabmodule}[0]{\operatorname{-\underline{gmod}}}

\newcommand{\stabgmodule}[0]{\operatorname{-\uli{gmod}}}
\newcommand{\stabgfmodule}[0]{\operatorname{-\uli{gfmod}}}
\newcommand{\gstabmodule}[0]{\operatorname{-\uli{gmod}}}


\newcommand{\comodule}[0]{\operatorname{-comod}}
\newcommand{\gcomodule}[0]{\operatorname{-gcomod}}
%% \newcommand{\stabcomodule}[0]{\operatorname{-\underline{comod}}}
%% \newcommand{\stabgcomodule}[0]{\operatorname{-\underline{gcomod}}}
%% \newcommand{\stabgcomod}[0]{\operatorname{-\underline{gcomod}}}

\newcommand{\stabcomodule}[0]{\operatorname{-\uli{comod}}}
\newcommand{\stabgcomodule}[0]{\operatorname{-\uli{gcomod}}}
\newcommand{\stabgcomod}[0]{\operatorname{-\uli{gcomod}}}


\newcommand{\antip}[0]{S}
\newcommand{\TTL}[0]{\widetilde{\TL}}
\newcommand{\cal}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\Mb}[1]{\ensuremath{\mathbb{#1}}}

\newcommand{\coneqnOne}[0]{(8.1)}
\newcommand{\coneqnTwo}[0]{(8.2)}

\newcommand{\normaltext}[1]{\textnormal{#1}}
\newcommand{\quantg}[0]{\Univ_q\mathfrak{g}}
\newcommand{\quantsl}[0]{\Univ_q\mathfrak{sl}(2)}
\newcommand{\cquantsl}[0]{\aU}
\newcommand{\cpquantsl}[0]{\aU^+}
\newcommand{\quantsu}[0]{\Univ_q\mathfrak{sl}(2)}
\newcommand{\quantso}[0]{\Univ_q\mathfrak{so}(3)}



\DeclareMathOperator{\Core}{\mathfrak{C}}
%\newcommand{\C}{\mathbb{C}}
%% \newcommand{\ZZ}{\mathbb{Z}}
%% \newcommand{\NN}{\mathbb{N}}
%% \newcommand{\FF}{\mathbb{F}}
%% \newcommand{\CC}{\mathbb{C}}
%% \newcommand{\Abb}{\mathbb{A}}
%% \newcommand{\PP}{\mathbb{P}}
%% \newcommand{\RR}{\mathbb{R}}
%% \newcommand{\QQ}{\mathbb{Q}}
%% \newcommand{\LL}{\mathbb{L}}
%% \newcommand{\GG}{\mathbb{G}}

%% \newcommand{\aA}{\mathcal{A}}
%% \newcommand{\aB}{\mathcal{B}}
%% \newcommand{\aW}{\mathcal{W}}
%% \newcommand{\aC}{\mathcal{C}}
%% \newcommand{\aD}{\mathcal{D}}
%% \newcommand{\aE}{\mathcal{E}}
%% \newcommand{\aF}{\mathcal{F}}
%% \newcommand{\aM}{\mathcal{M}}
%% \newcommand{\aV}{\mathcal{V}}
%% \newcommand{\aK}{\mathcal{K}}
%% \newcommand{\aG}{\mathcal{G}}
%% \newcommand{\aN}{\mathcal{N}}
%% \newcommand{\aP}{\mathcal{P}}
%% \newcommand{\aR}{\mathcal{R}}
%% \newcommand{\aI}{\mathcal{I}}
%% \newcommand{\aU}{\mathcal{U}}
%% \newcommand{\aL}{\mathcal{L}}
%% \newcommand{\aO}{\mathcal{O}}
%% \newcommand{\aS}{\mathcal{S}}
%% \newcommand{\aT}{\mathcal{T}}
%% \newcommand{\aQ}{\mathcal{Q}}

%% \newcommand{\mfF}{\mathfrak{f}}
%% \newcommand{\mfG}{\mathfrak{g}}
%% \newcommand{\mfH}{\mathfrak{h}}

\newcommand{\scrD}{\mathscr{D}}
\newcommand{\scrU}{\mathscr{U}}
\newcommand{\Nil}{\mathscr{N}\!{\it il}}
%\newcommand{\Nil}{\aN\!{\it il}}
\newcommand{\UmodNil}{\scrU\!/\!\Nil}
\newcommand{\mar}[0]{\aM}

% \newcommand{\sat}[0]{\ensuremath{\aA_2}}
% \newcommand{\sap}[0]{\ensuremath{\aA_p}}
% \newcommand{\ssat}[1]{\ensuremath{\aA_2(#1)}}
% \newcommand{\ssap}[1]{\ensuremath{\aA_p(#1)}}
% \newcommand{\dsat}[0]{\ensuremath{\aA^2}}
% \newcommand{\dsap}[0]{\ensuremath{\aA^p}}
% \newcommand{\dssats}[1]{\ensuremath{\aA^2(#1)}}
% \newcommand{\dssap}[1]{\ensuremath{\aA^p(#1)}}



\makeatletter
\def\imod#1{\allowbreak\mkern2.5mu({\operator@font mod}\,#1)}
\makeatother

\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\e}{\epsilon}
\newcommand{\vp}{\varphi}
%\newcommand{\op}{\oplus}
\newcommand{\opp}{\oplus}
\newcommand{\ott}{\otimes}
\newcommand{\pp}{\phi}
\renewcommand{\l}{\lambda}
\newcommand{\s}{\sigma}
\renewcommand{\r}{\rho}
\newcommand{\De}{\Delta}
\newcommand{\Ga}{\Gamma}
\newcommand{\ga}{\gamma}
\renewcommand{\th}{\theta}
\renewcommand{\d}{\delta}
%\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\Fl}{Fl}
\DeclareMathOperator{\Flag}{Flag}
%\newcommand{\Z}{\mathbb{Z}}

\newcommand{\CPic}[1]{
\begin{minipage}{.45in}
\includegraphics[scale=.75]{#1}
\end{minipage}
}

\newcommand{\CPPic}[1]{
\begin{minipage}{.8in}
\includegraphics[scale=1.1]{#1}
\end{minipage}
}

\newcommand{\BCPPic}[1]{
\begin{minipage}{1.6in}
\includegraphics[scale=2]{#1}
\end{minipage}
}



\newcommand{\MPic}[1]{
\begin{minipage}{.35in}
\includegraphics[scale=.45]{#1}
\end{minipage}
}

\newcommand{\BPic}[1]{
\begin{minipage}{1in}
\includegraphics[scale=1.5]{#1}
\end{minipage}
}

\newcommand{\oPic}[1]{
\begin{minipage}{.2in}
\includegraphics[scale=.3]{#1}
\end{minipage}
}

\newcommand{\mPic}[1]{
\begin{minipage}{.15in}
\includegraphics[scale=.22]{#1}
\end{minipage}
 }


\newcommand{\SPic}[1]{
\begin{minipage}{.75in}
\includegraphics[scale=1.15]{#1}
\end{minipage}
}

\newcommand{\Cpic}{\CPic}
\newcommand{\Spic}{\SPic}
\newcommand{\Mpic}{\MPic}

% \newcommand{\ps}[1]{\llbracket #1 \rrbracket}
% \newcommand{\ul}[1]{\underline{#1}}
% \newcommand{\ol}[1]{\overline{#1}}
% \newcommand{\Ormf}{\ensuremath{R\ps{M}}}
% \newcommand{\rmff}{\ensuremath{R\ps{M}_F}}
% \newcommand{\rmfp}{\ensuremath{R[M]}}
% \newcommand{\rmffp}{\ensuremath{R[M]}}
% \newcommand{\rtff}{\ensuremath{R\ps{T_l}}}
% \newcommand{\rlf}{\ensuremath{R(l)_F}}
% \newcommand{\rmf}{\ensuremath{R(m)_F}}
% \newcommand{\rlmf}{\ensuremath{R(l+m)_F}}
% \newcommand{\rtf}{\ensuremath{R\ps{T_l}}}
% \newcommand{\symrtf}{\ensuremath{\Sym(R\ps{T_l})}}
% \newcommand{\symrlf}{\ensuremath{R(l)_F^W}}
% \newcommand{\symrmf}{\ensuremath{R(m)_F^W}}
% \newcommand{\symrlmf}{\ensuremath{R(l+m)_F^W}}
% \newcommand{\symrlg}{\ensuremath{R(l)_G^W}}
% \newcommand{\nhrlf}{\ensuremath{\NH(l)_F}}
% %\newcommand{\nhrle}{\ensuremath{\NH(l)_{|E}}}
% %\newcommand{\nhrme}{\ensuremath{\NH(m)_{|E}}}
% %\newcommand{\nhrlme}{\ensuremath{\NH(l+m)_{|E}}}
% \newcommand{\nhrmf}{\ensuremath{\NH(m)_F}}
% \newcommand{\nhrlmf}{\ensuremath{\NH(l+m)_F}}
% \newcommand{\dlf}{\ensuremath{\aD(l)_F}}
% \newcommand{\nhrtf}{\ensuremath{\NH(R\ps{T_l})}}
% \newcommand{\symrtff}{\ensuremath{\Sym(R\ps{T_l}_F)}}
% \newcommand{\symrmff}{\ensuremath{\Sym(R\ps{M}_F)}}
% \newcommand{\nhrtff}{\ensuremath{\NH(R\ps{T_l}_F)}}
% \newcommand{\nhrmff}{\ensuremath{\NH(R\ps{M}_F)}}

% regular calligraphics
\newcommand{\aA}{\mathcal{A}}
\newcommand{\aB}{\mathcal{B}}
\newcommand{\aC}{\mathcal{C}}
\newcommand{\aD}{\mathcal{D}}
\newcommand{\aE}{\mathcal{E}}
\newcommand{\aF}{\mathcal{F}}
\newcommand{\aG}{\mathcal{G}}
\newcommand{\aH}{\mathcal{H}}
\newcommand{\aI}{\mathcal{I}}
\newcommand{\aJ}{\mathcal{J}}
\newcommand{\aK}{\mathcal{K}}
\newcommand{\aL}{\mathcal{L}}
\newcommand{\aM}{\mathcal{M}}
\newcommand{\aN}{\mathcal{N}}
\newcommand{\aO}{\mathcal{O}}
\newcommand{\aP}{\mathcal{P}}
\newcommand{\aQ}{\mathcal{Q}}
\newcommand{\aR}{\mathcal{R}}
\newcommand{\aS}{\mathcal{S}}
\newcommand{\aT}{\mathcal{T}}
\newcommand{\aU}{\mathcal{U}}
\newcommand{\aV}{\mathcal{V}}
\newcommand{\aW}{\mathcal{W}}
\newcommand{\aX}{\mathcal{X}}
\newcommand{\aY}{\mathcal{Y}}
\newcommand{\aZ}{\mathcal{Z}}

%mathboldfont
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}


%uppercase frak
\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}

%lowercase frak
\newcommand{\fa}{\mathfrak{a}}
\newcommand{\fb}{\mathfrak{b}}
\newcommand{\fc}{\mathfrak{c}}
\newcommand{\fd}{\mathfrak{d}}
\newcommand{\fe}{\mathfrak{e}}
\newcommand{\ff}{\mathfrak{f}}
\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fh}{\mathfrak{h}}
\newcommand{\fii}{\mathfrak{i}}
\newcommand{\fj}{\mathfrak{j}}
\newcommand{\fk}{\mathfrak{k}}
\newcommand{\fl}{\mathfrak{l}}
\newcommand{\fm}{\mathfrak{m}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fo}{\mathfrak{o}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\fr}{\mathfrak{r}}
\newcommand{\fs}{\mathfrak{s}}
\newcommand{\ft}{\mathfrak{t}}
\newcommand{\fu}{\mathfrak{u}}
\newcommand{\fv}{\mathfrak{v}}
\newcommand{\fw}{\mathfrak{w}}
\newcommand{\fx}{\mathfrak{x}}
\newcommand{\fy}{\mathfrak{y}}
\newcommand{\fz}{\mathfrak{z}}

%text
\newcommand{\rA}{\mathrm{A}}
\newcommand{\rB}{\mathrm{B}}
\newcommand{\rC}{\mathrm{C}}
\newcommand{\rD}{\mathrm{D}}
\newcommand{\rE}{\mathrm{E}}
\newcommand{\rF}{\mathrm{F}}
\newcommand{\rG}{\mathrm{G}}
\newcommand{\rH}{\mathrm{H}}
\newcommand{\rI}{\mathrm{I}}
\newcommand{\rJ}{\mathrm{J}}
\newcommand{\rK}{\mathrm{K}}
\newcommand{\rL}{\mathrm{L}}
\newcommand{\rM}{\mathrm{M}}
\newcommand{\rN}{\mathrm{N}}
\newcommand{\rO}{\mathrm{O}}
\newcommand{\rP}{\mathrm{P}}
\newcommand{\rQ}{\mathrm{Q}}
\newcommand{\rR}{\mathrm{R}}
\newcommand{\rS}{\mathrm{S}}
\newcommand{\rT}{\mathrm{T}}
\newcommand{\rU}{\mathrm{U}}
\newcommand{\rV}{\mathrm{V}}
\newcommand{\rW}{\mathrm{W}}
\newcommand{\rX}{\mathrm{X}}
\newcommand{\rY}{\mathrm{Y}}
\newcommand{\rZ}{\mathrm{Z}}

%sans serif
\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}






%blackboard bbm
\usepackage{bbm}
\newcommand{\mAA}{\mathbbm{A}}
\newcommand{\mBB}{\mathbbm{B}}
\newcommand{\mCC}{\mathbbm{C}}
\newcommand{\mDD}{\mathbbm{D}}
\newcommand{\mEE}{\mathbbm{E}}
\newcommand{\mFF}{\mathbbm{F}}
\newcommand{\mGG}{\mathbbm{G}}
\newcommand{\mHH}{\mathbbm{H}}
\newcommand{\mII}{\mathbbm{I}}
\newcommand{\mJJ}{\mathbbm{J}}
\newcommand{\mKK}{\mathbbm{K}}
\newcommand{\mLL}{\mathbbm{L}}
\newcommand{\mMM}{\mathbbm{M}}
\newcommand{\mNN}{\mathbbm{N}}
\newcommand{\mOO}{\mathbbm{O}}
\newcommand{\mPP}{\mathbbm{P}}
\newcommand{\mQQ}{\mathbbm{Q}}
\newcommand{\mRR}{\mathbbm{R}}
\newcommand{\mSS}{\mathbbm{S}}
\newcommand{\mTT}{\mathbbm{T}}
\newcommand{\mUU}{\mathbbm{U}}
\newcommand{\mVV}{\mathbbm{V}}
\newcommand{\mWW}{\mathbbm{W}}
\newcommand{\mXX}{\mathbbm{X}}
\newcommand{\mYY}{\mathbbm{Y}}
\newcommand{\mZZ}{\mathbbm{Z}}

%ams mathbb
\renewcommand{\AA}{\mathbb{A}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}

\newcommand{\kk}{\mathbb{k}}

%zipf calligraphics
\newcommand{\eA}{\EuScript{A}}
\newcommand{\eB}{\EuScript{B}}
\newcommand{\eC}{\EuScript{C}}
\newcommand{\eD}{\EuScript{D}}
\newcommand{\eE}{\EuScript{E}}
\newcommand{\eF}{\EuScript{F}}
\newcommand{\eG}{\EuScript{G}}
\newcommand{\eH}{\EuScript{H}}
\newcommand{\eI}{\EuScript{I}}
\newcommand{\eJ}{\EuScript{J}}
\newcommand{\eK}{\EuScript{K}}
\newcommand{\eL}{\EuScript{L}}
\newcommand{\eM}{\EuScript{M}}
\newcommand{\eN}{\EuScript{N}}
\newcommand{\eO}{\EuScript{O}}
\newcommand{\eP}{\EuScript{P}}
\newcommand{\eQ}{\EuScript{Q}}
\newcommand{\eR}{\EuScript{R}}
\newcommand{\eS}{\EuScript{S}}
\newcommand{\eT}{\EuScript{T}}
\newcommand{\eU}{\EuScript{U}}
\newcommand{\eV}{\EuScript{V}}
\newcommand{\eW}{\EuScript{W}}
\newcommand{\eX}{\EuScript{X}}
\newcommand{\eY}{\EuScript{Y}}
\newcommand{\eZ}{\EuScript{Z}}






\theoremstyle{plain}

%****Peter: Old version here
%\newtheorem{thm}[subsection]{Theorem}
%\newtheorem{theorem}[subsection]{Theorem}
%****Peter: New version here
\newtheorem{thm}{Theorem}[section]
\newtheorem*{introthm}{Theorem}
\newtheorem{theorem}[thm]{Theorem}


%\newtheorem{theorem}[subsubsection]{Theorem}
\newtheorem{application}[thm]{Application}
%\newtheorem{example}{Example}
\newtheorem{question}[thm]{Question}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem*{introconjecture}{Conjecture}
\newtheorem{properties}[thm]{Properties}
\newtheorem{propertyy}[thm]{Property}
\newtheorem{upropertyy}[thm]{Universal property}
\newtheorem{axioms}[thm]{Axioms}

%****Peter: Old version here
%\newtheorem{proposition}[subsection]{Proposition}
%\newtheorem{prop}[subsection]{Proposition}
%\newtheorem{defprop}[subsection]{Definition-Proposition}
%%\newtheorem{proposition}[subsubsection]{Proposition}
%\newtheorem{corollary}[subsection]{Corollary}
%\newtheorem{cor}[subsection]{Corollary}
%%\newtheorem{corollary}[subsubsection]{Corollary}
%\newtheorem{lemma}[subsection]{Lemma}
%****Peter: new version here
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{defprop}[thm]{Definition-Proposition}
%\newtheorem{proposition}[subsubsection]{Proposition}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{cor}[thm]{Corollary}
%\newtheorem{corollary}[subsubsection]{Corollary}
\newtheorem{lemma}[thm]{Lemma}



%\newtheorem{lemma}[subsubsection]{Lemma}
\theoremstyle{remark}
\newtheorem{partt}[thm]{Part}
\newtheorem*{comment}{Comment}
%\newtheorem{remark}[subsubsection]{Remark}


%****Peter: OLd version
%\newtheorem{warning}[subsection]{Warning}
%\newtheorem{obiterdictum}[subsection]{Obiter Dictum}
%\newtheorem{observation}[subsection]{Observation}
\newtheorem{warning}[thm]{Warning}
\newtheorem{obiterdictum}[thm]{Obiter Dictum}
\newtheorem{observation}[thm]{Observation}

%\newtheorem{observation}[subsubsection]{Observation}
\theoremstyle{definition}

%****Peter: Old version
%\newtheorem{example}[subsection]{Example}
%%\newtheorem{example}[subsubsection]{Example}
%\newtheorem*{problem}{Problem}
%\newtheorem{defn}[subsection]{Definition}
%\newtheorem{definition}[subsection]{Definition}
%%\newtheorem{definition}[subsubsection]{Definition}
%\newtheorem{variations}[subsection]{Variations}
%%\newtheorem{variations}[subsubsection]{Variations}
%\newtheorem*{claim}{Claim}
%\newtheorem*{answer}{Answer}
%\newtheorem{notation}[subsection]{Notation}
%\newtheorem{rmk}[subsection]{Remark}
%\newtheorem{remark}[subsection]{Remark}
%%\newtheorem{notation}[subsubsection]{Notation}
%\newtheorem*{terminology}{Terminology}
%\numberwithin{equation}{section}
\newtheorem{example}[thm]{Example}
%\newtheorem{example}[subsubsection]{Example}
\newtheorem*{problem}{Problem}
\newtheorem{defn}[thm]{Definition}
\newtheorem*{introdefn}{Definition}
\newtheorem{definition}[thm]{Definition}
%\newtheorem{definition}[subsubsection]{Definition}
\newtheorem{variations}[thm]{Variations}
%\newtheorem{variations}[subsubsection]{Variations}
\newtheorem{claim}[thm]{Claim}
\newtheorem{answer}[thm]{Answer}
\newtheorem{notation}[thm]{Notation}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
%\newtheorem{notation}[subsubsection]{Notation}
\newtheorem{terminology}[thm]{Terminology}
\numberwithin{equation}{section}


==> final submit/mypackages.tex <==
\usepackage{amsmath, amscd, amssymb, amsthm,amsfonts}
\usepackage{stmaryrd,euscript, mathrsfs, latexsym,mathabx}
\usepackage{color}
\usepackage{hyperref} % links to refs
%\usepackage{diagrams}

\usepackage{lmodern}
\usepackage[T1]{fontenc} % things like \"o
%\usepackage{tipa}

\usepackage{multicol}

\ifx\pdfoutput\undefined
\usepackage{graphicx}
\else
\fi

\ifx\xetex
\usepackage{fontspec}
\usefont{EU1}{lmr}{m}{n}%Latin Modern in OpenType format.
%\usefont{T1}{lmr}{m}{n}%Latin Modern in Type 1 format.
\else
\fi

\usepackage{url} % hyperref works too
\urlstyle{same}  % (sf also works, for something more subtle than tt)

% tikz diagrams
\usepackage{tikz}
\usetikzlibrary{matrix,arrows,positioning}
\tikzset{node distance=2cm, auto}

%datetime
\usepackage[nodayofweek]{datetime}

% microtype fancy options

\pdfoutput=1
\usepackage[activate={true,nocompatibility},final,kerning=true,tracking=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}
\SetTracking{encoding={*}, shape=sc}{0}
\microtypecontext{spacing=nonfrench}

 \mathsurround=1pt
 \footskip=4ex 

% %\parskip=6pt plus3pt minus3pt
% %\lineskip=1.25pt
% %\textwidth=6.5in 
% %\textheight=9in
% %\usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}

\textwidth 17cm
\oddsidemargin -0.3cm
\evensidemargin -0.3cm

%\usepackage[margin=1in]{geometry}

%\parskip=6pt plus3pt minus3pt

\baselineskip=14pt
%\def\baselinestretch{1.2}       % magnification for line spacing
%\lineskip=0pt
\parskip=\medskipamount
%\lineskip=1.25pt
\def\baselinestretch{1.06}       % magnification for line spacing








%krushkal
\headheight=7pt \topmargin=4pt \textheight=604pt \textwidth=432pt
\oddsidemargin=18pt \evensidemargin=18pt \flushbottom
%\setlength{\parindent}{0pt}
%\setlength{\parskip}{6pt plus3pt minus3pt}

\setlength{\mathsurround}{1pt}







\flushbottom





% % space above equation (either)
 \abovedisplayskip=1em plus.3em minus.5em
% % " below
 \belowdisplayskip=1em plus.3em minus.5em
% % " above when no overlap
 \abovedisplayshortskip=.5em plus.2em minus.4em
% % " below
 \belowdisplayshortskip=.5em plus.2em minus.4em

\pagestyle{plain}



% Only sections appear in table of contents.
\setcounter{tocdepth}{1}
% Don't force the bottoms of the pages to be at the same spot:
\raggedbottom
% Allow worse line breaks while this work is in progress.
\tolerance=3000
% We'll get fewer ``underfull hbox'' messages with this set.
\hbadness=4000
% We'll get fewer ``overfull hbox'' messages with this set.
\hfuzz=1pt





